Callipepla: Stream Centric Instruction Set and Mixed Precision for Accelerating Conjugate Gradient Solver

The continued growth in the processing power of FPGAs coupled with high bandwidth memories (HBM), makes systems like the Xilinx U280 credible platforms for linear solvers which often dominate the run time of scientific and engineering applications. In this paper, we present Callipepla, an accelerator for a preconditioned conjugate gradient linear solver (CG). FPGA acceleration of CG faces three challenges: (1) how to support an arbitrary problem and terminate acceleration processing on the fly, (2) how to coordinate long-vector data flow among processing modules, and (3) how to save off-chip memory bandwidth and maintain double (FP64) precision accuracy. To tackle the three challenges, we present (1) a stream-centric instruction set for efficient streaming processing and control, (2) vector streaming reuse (VSR) and decentralized vector flow scheduling to coordinate vector data flow among modules and further reduce off-chip memory accesses with a double memory channel design, and (3) a mixed precision scheme to save bandwidth yet still achieve effective double precision quality solutions. To the best of our knowledge, this is the first work to introduce the concept of VSR for data reusing between on-chip modules to reduce unnecessary off-chip accesses for FPGA accelerators. We prototype the accelerator on a Xilinx U280 HBM FPGA. Our evaluation shows that compared to the Xilinx HPC product, the XcgSolver, Callipepla achieves a speedup of 3.94x, 3.36x higher throughput, and 2.94x better energy efficiency. Compared to an NVIDIA A100 GPU which has 4x the memory bandwidth of Callipepla, we still achieve 77% of its throughput with 3.34x higher energy efficiency. The code is available at https://github.com/UCLA-VAST/Callipepla.

==> section/idea.tex <==
We address the challenges and questions raised in Section~\ref{sec:accchallenge}
with intuitions and inspirations in this section.

\subsection{Stream Based Instruction Set}
We design a stream based instruction set
to control the processing modules and 
data flows in the accelerators.
We encode vector and matrix
size and data flow directions in the
instruction. Therefore, we are able
so support an arbitrary problem for JPCGS
and
terminate the accelerator.
There are three principles for designing
our stream based instruction set: 
\begin{itemize}
\item \textbf{(1) Stream centric.} Every instruction is to process some streams.
JPCGS is dealing with vectors 
and matrices and we transfer them in streams.
Stream centric principle naturally enables
task parallelism.
\item \textbf{(2) Instruction triggered processing.} We use an instruction to trigger
the execution of a processing module which will either procure or consume streams.
\item \textbf{(3) Decoupled memory and computing.} We separate the memory load/store
from computation. In this way, we can benefit from pref etching and overlapped computing and memory accessing.
\end{itemize}

\begin{comment}
\begin{listing}[tb]
  \caption{Default vector add and the vector add in \calli.}
  \label{lst:vadd}
  \inputminted{cpp}{code/vadd.cpp}
\end{listing}
\end{comment}



\begin{comment}
We show a vector-add example in Code~\ref{code:vecadd}. We uses
three modules: a \texttt{Load} for loading a vector sending to a stream, a \texttt{Store}, and and an \texttt{Add}
 \begin{mycode}[tb]
    \centering
\includegraphics[width=1.0\columnwidth]{figure/C1.pdf}
	\vspace{-18pt}
	\caption{Default vector add and the vector add in \calli.}
	\vspace{-12pt}
	\label{code:vecadd}
\end{mycode}
\end{comment}


\subsection{Decentralized Vector Scheduling}

==> table/backup_resource.tex <==
 \begin{comment}
  \begin{tabular}{cccc}
    \hline
    & \textbf{xCGsolver} & \textbf{\calli-b} & \textbf{\calli}\\
    \hline

    LUT & 
    503K (38.6\%) & 
    399K (30.6\%) & 
    509K (38.9\%) 
    \\
    FF  & 
    878K (33.7\%) & 
    445K (17.1\%) & 
    557K (21.4\%) 
    \\
    DSP & 
    1196 (13.3\%) &
    1236 (13.7\%) &
    1940 (21.5\%) 
    \\
    BRAM & 
    595 (29.5\%) &
    460 (22.8\%) &
    716 (35.5\%) 
    \\
    URAM & 
    128 (13.3\%) &
    384 (40.0\%) &
    384 (40.0\%)
    \\
    \hline
  \end{tabular}
  \end{comment}
